Which Style Makes Me Attractive? Interpretable Control Discovery and Counterfactual Explanation on StyleGAN

The semantically disentangled latent subspace in GAN provides rich interpretable controls in image generation. This paper includes two contributions on semantic latent subspace analysis in the scenario of face generation using StyleGAN2. First, we propose a novel approach to disentangle latent subspace semantics by exploiting existing face analysis models, e.g., face parsers and face landmark detectors. These models provide the flexibility to construct various criterions with very concrete and interpretable semantic meanings (e.g., change face shape or change skin color) to restrict latent subspace disentanglement. Rich latent space controls unknown previously can be discovered using the constructed criterions. Second, we propose a new perspective to explain the behavior of a CNN classifier by generating counterfactuals in the interpretable latent subspaces we discovered. This explanation helps reveal whether the classifier learns semantics as intended. Experiments on various disentanglement criterions demonstrate the effectiveness of our approach. We believe this approach contributes to both areas of image manipulation and counterfactual explainability of CNNs. The code is available at \url{https://github.com/prclibo/ice}.

==> PaperForReviewaux.tex <==



==> figs/subspace_viz/short.tex <==

\begin{tikzpicture}
\footnotesize


\node[inner sep=0,outer sep=0] (skin0) {\includegraphics[width=0.19\textwidth]{figs/subspace_viz/face_color/r0_b0_v0.pdf}};
\node[fill=white, below=1pt of skin0.north] {Black/white};
\node[right=1.6pt of skin0.east, inner sep=0,outer sep=0] (skin1) {\includegraphics[width=0.19\textwidth]{figs/subspace_viz/face_color/r0_b0_v0.pdf}};
\node[fill=white, below=1pt of skin1.north] {Black/white};
\node[right=1.6pt of skin1.east, inner sep=0,outer sep=0] (skin2) {\includegraphics[width=0.19\textwidth]{figs/subspace_viz/face_color/r0_b0_v0.pdf}};
\node[fill=white, below=1pt of skin2.north] {Black/white};
\node[right=1.6pt of skin2.east, inner sep=0,outer sep=0] (skin3) {\includegraphics[width=0.19\textwidth]{figs/subspace_viz/face_color/r0_b0_v0.pdf}};
\node[fill=white, below=1pt of skin3.north] {Black/white};
\node[right=1.6pt of skin3.east, inner sep=0,outer sep=0] (skin4) {\includegraphics[width=0.19\textwidth]{figs/subspace_viz/face_color/r0_b0_v0.pdf}};
\node[fill=white, below=1pt of skin4.north] {Black/white};
\node[left=0.1cm of skin0.west]{\rotatebox{90}{Skin color}};

\node[below=2pt of skin0.south, inner sep=0,outer sep=0] (mshape0) {\includegraphics[width=0.19\textwidth]{figs/subspace_viz/face_color/r0_b0_v0.pdf}};
\node[fill=white, below=1pt of mshape0.north] {Black/white};
\node[right=1.6pt of mshape0.east, inner sep=0,outer sep=0] (mshape1) {\includegraphics[width=0.19\textwidth]{figs/subspace_viz/face_color/r0_b0_v0.pdf}};
\node[fill=white, below=1pt of mshape1.north] {Black/white};
\node[right=1.6pt of mshape1.east, inner sep=0,outer sep=0] (mshape2) {\includegraphics[width=0.19\textwidth]{figs/subspace_viz/face_color/r0_b0_v0.pdf}};
\node[fill=white, below=1pt of mshape2.north] {Black/white};
\node[right=1.6pt of mshape2.east, inner sep=0,outer sep=0] (mshape3) {\includegraphics[width=0.19\textwidth]{figs/subspace_viz/face_color/r0_b0_v0.pdf}};
\node[fill=white, below=1pt of mshape3.north] {Black/white};
\node[right=1.6pt of mshape3.east, inner sep=0,outer sep=0] (mshape4) {\includegraphics[width=0.19\textwidth]{figs/subspace_viz/face_color/r0_b0_v0.pdf}};
\node[fill=white, below=1pt of mshape4.north] {Black/white};
\node[left=0.1cm of mshape0.west]{\rotatebox{90}{Skin color}};

\node[below=2pt of mshape0.south, inner sep=0,outer sep=0] (mshapeid0) {\includegraphics[width=0.19\textwidth]{figs/subspace_viz/face_color/r0_b0_v0.pdf}};
\node[fill=white, below=1pt of mshapeid0.north] {Black/white};
\node[right=1.6pt of mshapeid0.east, inner sep=0,outer sep=0] (mshapeid1) {\includegraphics[width=0.19\textwidth]{figs/subspace_viz/face_color/r0_b0_v0.pdf}};
\node[fill=white, below=1pt of mshapeid1.north] {Black/white};
\node[right=1.6pt of mshapeid1.east, inner sep=0,outer sep=0] (mshapeid2) {\includegraphics[width=0.19\textwidth]{figs/subspace_viz/face_color/r0_b0_v0.pdf}};
\node[fill=white, below=1pt of mshapeid2.north] {Black/white};
\node[right=1.6pt of mshapeid2.east, inner sep=0,outer sep=0] (mshapeid3) {\includegraphics[width=0.19\textwidth]{figs/subspace_viz/face_color/r0_b0_v0.pdf}};
\node[fill=white, below=1pt of mshapeid3.north] {Black/white};
\node[right=1.6pt of mshapeid3.east, inner sep=0,outer sep=0] (mshapeid4) {\includegraphics[width=0.19\textwidth]{figs/subspace_viz/face_color/r0_b0_v0.pdf}};
\node[fill=white, below=1pt of mshapeid4.north] {Black/white};
\node[left=0.1cm of mshapeid0.west]{\rotatebox{90}{Skin color}};

\end{tikzpicture}


==> supaux.tex <==


